Performance and optimization of support vector machines in high-energy physics classification problems

In this paper we promote the use of Support Vector Machines (SVM) as a machine learning tool for searches in high-energy physics. As an example for a new- physics search we discuss the popular case of Supersymmetry at the Large Hadron Collider. We demonstrate that the SVM is a valuable tool and show that an automated discovery- significance based optimization of the SVM hyper-parameters is a highly efficient way to prepare an SVM for such applications. A new C++ LIBSVM interface called SVM-HINT is developed and available on Github.

==> Implementations.tex <==
% !TEX root = svm_paper.tex

\section{Implementations}\label{sec:classimp}
Modern high-energy physics (HEP) collider experiments pose a great challenge for physicists in terms of analysis and classification of the collected data or the simulated samples. 
The ROOT analysis framework is widely used among high energy physicists to overcome some of these challenges of HEP collider experiments. Very rare processes of interests (in the following called 'signal') need to be separated from a large sample of background events. Therefore, physicists can benefit strongly from machine learning techniques like SVM and BDT. For this purpose we developed a new ROOT interface to LIBSVM. In the following we compare the performance and ease of use of the new LIBSVM-ROOT interface with the popular HEP multivariate analysis toolkit TMVA. The BDT implementation of the TMVA package is used as a reference of performance comparison since it is very popular among experimental HEP physicists and claimed to be one of the best out-of-the-box classifiers. 
In the TMVA version used in this paper (4.2.0), the SVM implementation includes only the RBF kernel, while the LIBSVM's implementation accompanies RBF, polynomial, sigmoidal, and linear kernels. Unlike TMVA, LIBSVM also contains different soft margin approaches. However, these differences are irrelevant to the context of the performance comparison.  On the other hand, these two SVM implementations are expected to differ in performance due to different sequential minimal optimization methods followed in the minimization problem. Neither of these two packages have built in hyper-parameter search functionality, however, an external grid search script is available on the LIBSVM webpage. TMVA offers a more complete framework, yet the trade off is a very closed environment, which makes individual TMVA classifiers harder to use outside of the TMVA framework. Therefore, in terms of ease of development, LIBSVM is used to develop the interface.\\
\subsection{SVM-HINT}
The SVM-HINT is a C++11 based classifier interface to make the LIBSVM software package developed for the high energy physics classification applications accompanying a statistical significance based; powerful and fast autonomous hyper parameter search implementation. The SVM-HINT uses LIBSVM and the ROOT libraries to provide fast and easy to use binary classifier application. After background and signal samples being set by user, SVM-HINT employs the custom hyper-parameter grid search algorithm described in the appendix \ref{app:itergrid} to obtain the optimum hyper-parameters. These parameters are then used in the evaluation sample to obtain the final classification. The SVM-HINT uses built in open MP support of the LIBSVM and also accompanies it with a multi-threaded significance comparison for the test samples. Using operating-software dependent functions to adjust the thread numbers, SVM-HINT can run faster in multi-threaded environments out of the box. \\
Currently the SVM-HINT supports the SVM classifier with the slack variable $C$ for binary classification problems. Since it is designed as an abstract factory class, other implementations can be added easily as well. 

\subsection{TMVA}
\subsubsection{Boosted Decision Trees}\label{BDT2}
DK: to be shortened
\paragraph{Binary Decision Trees}\label{BDT3}
!!! For this part out main reference should definitely be Classification and Regression Trees, Breiman, Friedman, Olshen, Stone and for the Boosting (adaboost) Freund and Schapire's paper !!!
The binary decision trees are one of the most commonly used classifiers in experimental particle physics. Each node of a binary decision tree is connected to two branches that are split with respect to a feature. The decision of the feature and its cut value is adjusted by a performance measure. Since  even for relatively small sized trees, simultaneously calculating all possible combinations of a given feature set to obtain the optimal separation is a lengthy calculation, a node based adjustment is mainly followed. For each node, the optimal feature and its cut value are obtained by calculating each possible variation in the feature set and then ranking according to the performance measure. Therefore, each branch leads to a different optimized cubical separation in multi-dimensional feature space. The Gini index of diversity is used as the performance measure in this paper given by: 
!!! here the selection of the performance measure does not affect the result to much -  Gini index is the default of TMVA and it is one of few mentioned in the main reference (CART). Also in page 102 it is preferred for two-class problem !!!
%\begin{figure}[t] 
%\centering
%\includegraphics[width=0.4\textwidth]{figure_bdt.png}
%\caption{Representation of a simple binary decision tree structure: Each node is split with respect to a feature $\Theta_i$ and a cut value $\theta_i$ determined by the performance measure.}
%\label{fig:bdt}
%\end{figure}
\begin{equation}
i(t) = \sum\limits_{i \neq j} p(i|t) p(j|t)
\end{equation}
where $p(y|t)$ is the proportion of the class $y$ in the given node $t$. Therefore for the binary trees, it can be written as:
\begin{equation}
i(t) = p(y|t) (1-p(y|t))
\end{equation}
One of the most important challenges of decision trees is the determination of the node depth (adding new nodes to the tree). The method followed in this paper is allowing trees to grow as much as possible by respecting a minimum node size and, after growth, pruning branches which increase the misclassification cost. 
 There are multiple different ways of enhancing the performance of binary decision trees. In this paper, we focus on binary decision trees with boosting algorithm. Therefore, the abbreviation {\it BDT} is used for boosted binary decision trees. 
\paragraph{Boosting}
Boosting is a powerful iterative algorithm which improves the performance of base (or weak) classifiers. After each training of the base algorithm, boosting increases the weights of the misclassified training points. After the final iteration, each classifier contributes to the final decision proportional to its accuracy. The AdaBoost algorithm developed by Freund and Schapire is used in this paper. 
For the training set as defined in Equation~\ref{for:tra}, it can be summarized as follows:
\begin{enumerate}
\item For the first iteration, initialize the same weight for each training event: $D_1(i)=1/l$.
\item Train the base classifier on the weighted distribution $D_n$.
%%\item Correctly identified events keep the same weight, whereas the misclassified events weighted proportional to the misclassification rate of the weak classifier in given iteration.
\item Calculate the importance $\alpha_{n}$ of the given base classifier by evaluating 
\begin{equation}
\alpha_n = \frac{1}{2} \ln\left( \frac{1-\epsilon_n}{\epsilon_n}\right),
\end{equation}
where $\epsilon_n$ is the ratio of the misclassified events for the $n$th base classifier.
\item Update the weight distribution $D_{n+1}$
\begin{equation}
 D_{n+1}(i)=\frac{D_{n}(i) e^{\alpha_n y_n}}{Z_n},
\end{equation}
where $Z_n$ is the normalization factor.
\item Finally each weak classifier contributes to the final decision according to the classification performance obtained in each iteration:
\begin{equation}
Y(x) = sign\left(\sum \limits_{n} \alpha_n y_n(x)\right)
\end{equation}
\end {enumerate}

